Make It Make Sense! Understanding and Facilitating Sensemaking in Computational Notebooks

Reusing and making sense of other scientists' computational notebooks. However, making sense of existing notebooks is a struggle, as these reference notebooks are often exploratory, have messy structures, include multiple alternatives, and have little explanation. To help mitigate these issues, we developed a catalog of cognitive tasks associated with the sensemaking process. Utilizing this catalog, we introduce Porpoise: an interactive overlay on computational notebooks. Porpoise integrates computational notebook features with digital design, grouping cells into labeled sections that can be expanded, collapsed, or annotated for improved sensemaking. We investigated data scientists' needs with unfamiliar computational notebooks and investigated the impact of Porpoise adaptations on their comprehension process. Our counterbalanced study with 24 data scientists found Porpoise enhanced code comprehension, making the experience more akin to reading a book, with one participant describing it as It's really like reading a book.

==> tables/Codebook.tex <==
\begin{flushleft}
\begin{table*}[t!]
\centering  % used for centering table
\caption{Categorization of Data science code tokens based on functions. \label{table:ds_functions}} % title of Table
 % is used to refer this table in the text
\begin{tabular}{lll}
\rowcolor[HTML]{FFFFFF} 
\textbf{Main category} & \textbf{Sub-category}   & \textbf{Defintion}                                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
Load (L)               & import/generate (L1)    & generating/importing data/packages                                 \\
                       & fetch/load (L2)         & loading datasets from local or cloud                               \\
\rowcolor[HTML]{EFEFEF} 
                       & inspect (L3)            & inspect data loade (print)                                         \\
                       & export (L4)             & export data created/obtained                                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
Special Operations(S)  & nlp operations (S1)     & using nlp packages to process text data                            \\
                       & querying (S2)           & using packages to query/select subset                              \\
\rowcolor[HTML]{EFEFEF} 
                       & parsing(S3)             & parse text, image, or sound data                                   \\
                       & math/sci (S4)           & define mathematical/scientific formulas                            \\
\rowcolor[HTML]{EFEFEF} 
                       & domain specific (S5)    & use very specific packages like map API                            \\
                       & image processing (S6)   & operating on images using packages                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
Pre-Process(PP)        & tidying data (PP1)      & cleaning and reshaping data                                        \\
                       & transforming data (PP2) & transforming data value or type                                    \\
\rowcolor[HTML]{EFEFEF} 
                       & formatting data (PP3)   & change the data format/shape (subset)                              \\
                       & summary (PP4)           & generate or print data summaries                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
Visualization(V)       & Distribution (V1)       & plot the distribution of data (histogram)                          \\
 & Relational (V2) & visualize the distribution between variables of the same data or different data \\
\rowcolor[HTML]{EFEFEF} 
                       & Comparative (V3)        & visualize different data using similar plots to compare data       \\
                       & Adjust (V4)             & adjust a previously created visualization                          \\
\rowcolor[HTML]{EFEFEF} 
                       & Output (V5)             & visualize the output of a model (regression, ML models, etc)       \\ \hline
Machine Learning(ML)   & Prep (ML1)              & prepare/define the models or set up a model                        \\
\rowcolor[HTML]{EFEFEF} 
                       & Train (ML2)             & training the model                                                 \\
                       & Test (ML3)              & test the output of the model                                       \\
\rowcolor[HTML]{EFEFEF} 
                       & Verify (ML4)            & print and verify the output of the model eg. error rates, accuracy \\
                       & Clustering (ML5)        & perform clustering on data                                         \\
\rowcolor[HTML]{EFEFEF} 
                       & Featuring (ML6)         & perform feature engineering on data                                \\
                       & Tuning (ML7)            & tuning the hyperparameters of a model                              \\
\rowcolor[HTML]{EFEFEF} 
                       & Special (ML8)           & perform functions to improve performance (ensemble, stacking, etc) \\ \hline
Statistics(ST)         & Summary (ST1)           & generate/print statistical summary measures                        \\
\rowcolor[HTML]{EFEFEF} 
                       & Measure (ST2)           & generate/print different statistical measures                      \\
                       & Plot (ST3)              & special cases of gaining statistical inference through plots       \\
\rowcolor[HTML]{EFEFEF} 
                       & Test (ST4)              & running statistical tests                                          \\
                       & Model (ST5)             & defining and running statistical models                            \\ \hline
\end{tabular}
\end{table*}
\end{flushleft}



==> tables/Codebook1.tex <==
\begin{table}[th!]
\caption{Categorization of code functionality}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llllll}
\rowcolor[HTML]{EFEFEF} 
\textbf{Load (L)} & \textbf{Pre-Process (PP)} & \textbf{Statistics (ST)} & \textbf{Visualization (V)} & \textbf{Domain Specific Functions (S)} & \textbf{Machine Leraning (ML)} \\ \hline
Import/generate (L1) & String operations (PP0) & Summary (ST1) & Distribution (V1) & NLP operations (S1) & Prep (ML1) \\
\rowcolor[HTML]{EFEFEF} 
Fetch/Load (L2) & Tidying data (PP1) & Measure (ST2) & Relational (V2) & Querying (S2) & Train (ML2) \\
Parsing (L3) & Transforming data (PP2) & Plot (ST3) & Comparative (V3) & Math/sci (S3) & Test (ML3) \\
\rowcolor[HTML]{EFEFEF} 
Export (L4) & Formatting data (PP3) & Test (ST4) & Modify visualization (V4) & Domain specific function (S4) & Verify (ML4) \\
 & Summary (PP4) & Model (ST5) & ML visualization (V5) & Image processing (S5) & Clustering (ML5) \\
\rowcolor[HTML]{EFEFEF} 
 & Data inspection(PP5) &  &  &  & Featuring (ML6) \\
 &  &  &  &  & Tuning (ML7) \\
\rowcolor[HTML]{EFEFEF} 
 &  &  &  &  & Special (ML8)
\end{tabular}}
\label{tab:ds_functions}
\end{table}

==> tables/Patterns.tex <==
\begin{table*}[t!]
\caption{Code purpose from functionality patterns in notebooks} 
\renewcommand{\arraystretch}{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll}
\textbf{Code Purpose} & \textbf{Description} \\
Libraries and system setup & The process of configuring a programming system libraries \\
Initial wrangling and data generation & \begin{tabular}[c]{@{}l@{}}Loading multiple data sources or generating a population, and tuning the data right\\ away based on what they know about the data.\end{tabular} \\
Domain specific wrangling & \begin{tabular}[c]{@{}l@{}}Loading and processing specific types of data like image, audio, geographical, or text. \\ Involves specific libraries and specific functional transformations.\end{tabular} \\
Inspection based transformation & \begin{tabular}[c]{@{}l@{}}Data is processed/changed, inspected in textual or visual form, followed by more changes \\ to the data.\end{tabular} \\
Initial visual inspection & Exploratory visual inspection of the data right after loading. \\
Summary based transformation & Inspection of summary measures that leads to certain transformations. \\
Feedback based selection & Select a different model based on the output metrics of the model. \\
Modelling with defaults & \begin{tabular}[c]{@{}l@{}}Models based on the team/organization, or models that were pre-trained, or with default parameters\\ with no tuning/training.\end{tabular} \\
AutoML by hand & \begin{tabular}[c]{@{}l@{}}Selecting among multiple models. Typically either all models are initiated at the same time, or they \\ are run one after the other.\end{tabular} \\
Parameter tuning & \begin{tabular}[c]{@{}l@{}}When the same model is refined by changing the parameters, or model structure, based on the result \\ of the model's output.\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Best practice based \\ transformation\end{tabular} & \begin{tabular}[c]{@{}l@{}}When standard processes are followed to tackle specific performance issues with the model. These \\ are handed down cookbook steps to take e.g. use ensemble to reduce error in regression.\end{tabular} \\
Input tuning & Standard processing of data after finding data related issues causing model performance to deteriorate. \\
Generic modeling & Typical cycle of define, train, test of an ML model. \\
Statistical Modeling & Defining and executing a statistical model or performing statistical testing. \\
Saving intermediate progress & Saving a model state with parameters, or saving transformed data for reuse. \\
Pre-model inspection of data & Checking the shape and elements of data, in textual or graphical format, right before feeding it into the model. \\
Model output inspection & Using just a print of the metrics or the visualization of the model's output. \\
Inspection based scientific coding & Building functions and transformations with interleaved data check along the way. \\
Output verification & \begin{tabular}[c]{@{}l@{}}Multiple format inspection of a model's output or a transformation. Often also involves checking the \\ statistical summary.\end{tabular}
\end{tabular}}
\label{table:patterns}
\end{table*}


==> tables/control_analysis.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Perspective}                                  & \textbf{Dimension}                     & \textbf{Information Needs}                                      & \textbf{Example} & \textbf{Participants} \\ \hline
\multirow{5}{*}{\textbf{Comprehension}}               & \multirow{2}{*}{Behavior}              & What is the goal of analysis, parts of analysis, or code cells? & ""{[}P1{]}       & P1, P2, P3            \\ \cline{3-5} 
                                                      &                                        & What type of analysis is included in the notebook?              &                  &                       \\ \cline{2-5} 
                                                      & Comparision                            & How do I compare similar analysis and results?                  &                  &                       \\ \cline{2-5} 
                                                      & \multirow{2}{*}{Knowledge/familiarity} & How does the library/function affect the data and results?      &                  &                       \\ \cline{3-5} 
                                                      &                                        & What do these libraries/functions broadly do?                   &                  &                       \\ \hline
\multirow{2}{*}{\textbf{Context/Situation awareness}} & \multirow{2}{*}{Infereing Hypothesis}  & How do the hypotheses connect to the goal?                      &                  &                       \\ \cline{3-5} 
                                                      &                                        & How is the data and problem defined?                            &                  &                       \\ \hline
\multirow{3}{*}{\textbf{Mental Model/Mapping}}        & Navigation                             & Where am I?                                                     &                  &                       \\ \cline{2-5} 
                                                      & \multirow{2}{*}{Structure}             & How are the different stages of analysis related?               &                  &                       \\ \cline{3-5} 
                                                      &                                        & How long is the script/part?                                    &                  &                       \\ \hline
\end{tabular}}
\end{table}

==> tables/design_mapping_2.tex <==
\resizebox{\textwidth}{!}{
\caption{Design feature mapping
\label{table:mapping2}} 
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{lllllll}
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{4}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Design featuers}} \\ \hline 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Element}}} & \multicolumn{1}{l}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Cognitive task}}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Helping notebook users \\ comprehend analysis \\ overview of its structure \\ and purpose.\end{tabular}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Enable notebook users\\ to find relevant \\ information.\end{tabular}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Allowing easier \\ pathways for \\ logical understanding.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Allow notebook users \\ to build and share \\ explanations.\end{tabular} \\ 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Understanding Behavior (C1)} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{A}\protect  \protect\overviewLabelBig{D}\protect  \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{B}\protect \protect\overviewLabelBig{C}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect \\ 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Comparing Information (C2)} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{A}\protect  \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &  \\  
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Comprehension}}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Broadening Knowledge (C3)} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} &  \\ 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}Understanding Structure (C4)} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{B}\protect \protect\overviewLabelBig{C}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect \\ 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Mental Modelling}}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Mapping/Relating Elements \\ and Concepts (C5)\end{tabular}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect  \protect\overviewLabelBig{E}\protect} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} &  \\  
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Inferring hypothesis (C6)} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{B} \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Situational awareness}}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Inferring elements (C7)} & \multicolumn{1}{l}{\multirow{-9}{*}{\cellcolor[HTML]{FFFFFF}}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}\protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{D}\protect \protect\overviewLabelBig{E}\protect} & \protect\overviewLabelBig{A}\protect \protect\overviewLabelBig{B} \protect\overviewLabelBig{D}\protect \\ 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\protect\overviewLabelBig{A}\protect: Navigation panel; \protect\overviewLabelBig{B}\protect: Annotation; \protect\overviewLabelBig{C}\protect: export; \protect\overviewLabelBig{D}\protect: Chapter title and icon; \protect\overviewLabelBig{E}\protect: Section title;} \\ 
\end{tabular}}

==> tables/information_needs.tex <==

\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\rowcolor[HTML]{EFEFEF} 
\textbf{Cognitive task} & \textbf{Challenges} & \textbf{Examples} & \textbf{Participants} \\ \hline
\multicolumn{4}{c}{\textbf{E1. Comprehension}} \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \begin{tabular}[c]{@{}l@{}}What is the goal of analysis, parts \\ of analysis, or code cells?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I have no idea what they’re trying to do, it seems \\ like they’re trying to sort something. (P3)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2, P3, P4, P5, P6,\\ P7, P8, P9, P10, P11, \\ P12, CP1, CP2, CP3, \\ CP4, CP5, CP6, CP7, \\ CP8, CP9, CP10, CP11, \\ CP12\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Understanding Behavior (C1)} & \begin{tabular}[c]{@{}l@{}}What type of analysis is included \\ in the notebook?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I'm not sure how they draw this conclusion just \\ logically I filled this part is missing. (CP4)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2, P3, P5, P6, P7,\\ P9, P12, CP2, CP3, CP4, \\ CP6, CP7, CP8, CP9\\ CP12\end{tabular} \\
Comparing Information (C2) & \begin{tabular}[c]{@{}l@{}}How do I compare similar analysis \\ and results?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}what’s different between the {[}result{]} and the \\ {[}result{]}. (P4)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2 P3, P4, P5, P8,\\ P9, P12, CP1, CP2, CP6, \\ CP7, CP8, CP9\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \begin{tabular}[c]{@{}l@{}}How does the library/function affect \\ the data and results?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I'm not sure what this function does. (CP8)\\ I don't know it's setting. (CP2)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P5, P8, P9, P12, CP1, CP2,\\ CP5, CP7, CP8, CP10, CP11\\ CP12\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Broadening Knowledge (C3)} & \begin{tabular}[c]{@{}l@{}}What do these libraries/functions \\ broadly do?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I’m not familiar with what this {[}function{]} it \\ looks like they’re just plotting different. (P3)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2, P3, P4, P5, CP4, \\ CP6, CP8, CP9, CP10, \\ CP11, CP12\end{tabular} \\
\multicolumn{4}{c}{\textbf{E2. Mental modelling}} \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & Where am I? & \textit{\begin{tabular}[c]{@{}l@{}}So they’re doing cross-validation just because \\ that’s probably in where’s the split Oh, \\ I lost it. (P12)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2, P3, P4, P5, P6,\\ P7, P8, P9, P10, P11, \\ P12, CP1, CP4, CP6, \\ CP8, CP12\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Understanding Structure (C4)} & How long is the script/part? & \textit{\begin{tabular}[c]{@{}l@{}}I forgot some of the parts. I'm trying to \\ remember. (CP11)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P1, P2, P9, CP4, CP5,\\ CP8, CP11\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Mapping/Relating Elements and \\ Concepts (C5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}How are the different stages of analysis \\ related?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I'm just trying to like kind of figure out what they're \\ going from here to here. (CP12)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P3, P5, P8, P12, CP1, CP2, \\ CP4, CP5, CP6, CP9, CP12\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{4}{c}{\cellcolor[HTML]{EFEFEF}\textbf{E3. Situational awareness}} \\
Inferring hypothesis (C6) & \begin{tabular}[c]{@{}l@{}}How do the hypotheses connect \\ to the goal?\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}I am assuming this is cross-validation stuff so they \\ are trying to do cross validation. (P2)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P2, P8, P9, P11, P12\\ CP2, CP5, CP7, CP8, \\ CP9\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
Inferring elements (C7) & How is the data and problem defined? & \textit{\begin{tabular}[c]{@{}l@{}}I was hoping that there would be very clear demarcation. \\ But definitely, that wasn't there. (CP8)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}P2, P3, P4, P5, P12, \\ CP4, CP8, CP9, CP12\end{tabular}
\end{tabular}}

==> tables/interviewParticipants.tex <==
\begin{table}[htb]
\caption{Demographic information of interview participants}
\resizebox{3.5 in}{!}{
\begin{tabular}{llllll}
\rowcolor[HTML]{FFFFFF} 
\textbf{ID} & \textbf{Role} & \textbf{Industry} & \textbf{Exp. (Yrs)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
F1  & Cloud Soln. Architect & Cloud Computing          & 4  \\
\rowcolor[HTML]{FFFFFF} 
F2  & Data Scientist        & Business Analytics       & 3  \\
\rowcolor[HTML]{EFEFEF} 
F3  & Data Scientist        & Cloud Computing          & 4  \\
\rowcolor[HTML]{FFFFFF} 
F4  & Data Scientist        & Security                 & 10  \\
\rowcolor[HTML]{EFEFEF} 
F5  & Data Scientist        & Cloud Computing          & 4   \\
\rowcolor[HTML]{FFFFFF} 
F6  & Soln. Architect       & Development Tools        & 4  \\
\rowcolor[HTML]{EFEFEF} 
F7  & Database Architect    & Environmental Consulting & 6  \\
\rowcolor[HTML]{FFFFFF} 
F8  & Data Analyst          & Entertainment            & 7  \\
\rowcolor[HTML]{EFEFEF} 
F9  & Software Engineer     & Manufacturing            & 8   \\
\rowcolor[HTML]{FFFFFF} 
F10 & Data Analyst          & Finance                  & 5    \\
\rowcolor[HTML]{EFEFEF} 
F11 & Consultant            & Finance                  & 9   \\
\rowcolor[HTML]{FFFFFF} 
F12 & Consultant            & Finance                  & 15   \\
\rowcolor[HTML]{EFEFEF} 
F13 & Data Scientist        & Security                 & 10    \\
\rowcolor[HTML]{FFFFFF} 
F14 & Software Engineer     & Cloud Computing          & 9      \\
\rowcolor[HTML]{EFEFEF} 
F15 & Data Scientist        & Development Tools        & 5    \\ 
\end{tabular}}
\label{tab:interviewparticipants}
\end{table}

==> tables/sense_making_def.tex <==
\begin{table}[t!]
\caption{Sensemaking activities}
\label{table:sense_making}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llll}
\rowcolor[HTML]{EFEFEF} 
\textbf{Element} & \textbf{Definition} & \textbf{Cognitive task} & \textbf{References} \\ \hline
Comprehension (E1) & \begin{tabular}[c]{@{}l@{}}Comprehension includes reading symbols and associating meaning\\ to the symbols based on our existing knowledge to identify patterns\\ and behavior of systems, compare information, and broaden knowledge\\ and understanding.\end{tabular} & Understanding Behavior (C1) & \cite{woods1997automation, von1993code, bryant2011software, wang2003cognitive} \\
 &  & Comparing Information (C2) & \cite{ntuen2006cognitive, klein2006making} \\
 &  & Broadening Knowledge (C3) & \cite{snowden2011naturalizing, snowden1999story, borges2010learning, fiol1985organizational, wang2006layered} \\
\rowcolor[HTML]{EFEFEF} 
Mental modelling (E2) & \begin{tabular}[c]{@{}l@{}}Mental models are internal memory representations depicting states\\ of events related to ideas, declarative and procedural knowledge, and inferences\\ drawn linked to or expressed in terms of concepts, principles, and knowledge. \\ If no suitable schema is available, people might create mental models to generate \\ descriptions of system purpose and form explanations of system functioning\end{tabular} & Understanding Structure (C4) & \cite{johnson1989mental, rutherford1991models, rouse1986looking, moray1998identifying} \\
\rowcolor[HTML]{EFEFEF} 
 &  & \begin{tabular}[c]{@{}l@{}}Mapping/Relating Elements and \\ Concepts (C5)\end{tabular} & \cite{abel1998mental, johnson1989mental, langan2004mental, vosniadou199416, nersessian2002cognitive} \\
Contextual inferences (E3) & \begin{tabular}[c]{@{}l@{}}Contextual inferences is a person’s perception of important information\\ items in their present work environment and capacity to project the\\ future condition of these elements.\end{tabular} & Inferring hypothesis (C6) & \cite{tiemens1989cognitive, klein2007data, endsley2017toward} \\
 &  & Inferring elements (C7) & \cite{tiemens1989cognitive, klein2007data, endsley2017toward}
\end{tabular}}
\end{table}
